Coupling Physics Informed Neural Networks with External Solvers

The current work aims to incorporate physics-based loss in Physics Informed Neural Network (PINN) directly using the numerical residual obtained from the governing equation in any dicretized forward solver. PINN's major difficulties in coupling with external forward solvers arise from the inability to access the discretized form (Finite difference, finite volume, finite element, etc.) of the governing equation directly through the network and to include them in its computational graph. This poses a significant challenge to conventional automatic-differentiation-based derivative computation of physics-based loss terms concerning the neural network hyperparameters if gradient-based optimization techniques are adopted. Therefore, we propose modifying the physics-based loss term to account for the residual arising from the external solver and to compute the derivative required for the optimization machinery. The proposed methodologies are demonstrated on benchmark full-order and reduced-order systems.

==> Command.tex <==
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}

\def\a{{\bm a}}
\def\b{{\bm b}}
\def\d{{\bm d}}
\def\f{{\bm f}}
\def\g{{\bm g}}
\def\n{{\bm n}}
\def\u{{\bm u}}
\def\v{{\bm v}}
\def\w{{\bm w}}
\def\x{{\bm x}}
\def\P{{\bm P}}
\def\U{{\bm U}}
\def\X{{\bm X}}
\def\0{\boldsymbol{0}}
\def\ss{\boldsymbol{\sigma}}
\def\SS{\boldsymbol{\Sigma}}
\def\ee{\boldsymbol{\eta}}
\def\mubar{\overline{\mu}}
\def\ubar{\overline{\u}}
\def\vbar{\overline{\v}}
\def\vtilde{\tilde{\v}}
\def\wbar{\overline{\w}}
\def\qbar{\overline{q}}
\def\dt{\partial_t}
\def\bbf{\mathbf{b}}
\def\ebf{\mathbf{e}}
\def\fbf{\mathbf{f}}
\def\qbf{\mathbf{q}}
\def\pbf{\mathbf{p}}
\def\vbf{\mathbf{v}}
\def\ubf{\mathbf{u}}
\def\xbf{\mathbf{x}}
\def\ybf{\mathbf{y}}
\def\vbarbf{\overline{\vbf}}
\def\qbarbf{\overline{\qbf}}
\def\xbarbf{\overline{\xbf}}
\def\bbarbf{\overline{\bbf}}

\def\uh{\u_h}
\def\vh{\v_h}
\def\fh{\f_h}
\def\bh{\b_h}
\def\ph{p_h}
\def\qh{q_h}
\def\vbarh{\vbar_h}
\def\qbarh{\qbar_h}
\def\mubarh{\mubar_h}

\def\cl {\nonumber \\}
\def\el {\nonumber }

\newtheorem{rem}{Remark}[section]

\def\Jcp{J. Comp. Phys}
\def\Cmame{Comput. Methods Appl. Mech. Engrg.}
\def\Jmpa{J. Math. Pures Appl.}
\def\Mmmas{Math. Model Meth. Appl. Sci.}
\def\Siamsc{SIAM J. Sci. Comp.}

\newcommand{\bm}[1]{\mbox{\boldmath{$#1$}}}
\def\div{\nabla\cdot}
\def\grad{\nabla}
\def\grads{\grad^s}

%\topmargin      10mm 
%\evensidemargin 5mm \oddsidemargin  5mm
%\textwidth      150mm \textheight 200mm \frenchspacing \sloppy

%\def\baselinestretch{2} 

\newcommand{\anna}[2][cyan]{\emph{\textcolor{#1}{#2}}}
\newcommand{\rev}[2][red]{{\textcolor{#1}{#2}}}



% To quantify the ROM accuracy, all snapshots are reconstructed in time using ROM techniques and the $l^2$-norm relative error for each snapshot is computed considering again three different energy threshold as before.  We were interested to see the effect of Dataset Size, i.e. Train to Test Split Ratios in our comparison to check the error convergence with the respect to this ratio. To this aim three ratio were considered; in the first case 50$\%$ of dataset is used to train the model, then 70$\%$ and finally 90$\%$ each of them for three various energy threshold.     

==> Introduction.tex <==
\section{\bf{Introduction}}\label{sec:Intro}

Reduced order modelling \cite{rozza2022advanced,quarteroni2015reduced,benner2020model} for computational physics problems has gained
significant research focus in the past few decades. Usually, the computational effort of reduced-order model development involves two distinct stages - one is the offline stage where the high-fidelity simulation datasets are generated using high-performance computing (HPC) and the other one is the online stage which is performed using comparatively less powerful machines. Based on the learning methodology of the parametric space or unsteady dynamics,  the reduced order model can
be broadly classified into two categories, i.e. intrusive and non-intrusive reduced order model. In the intrusive approach, the governing equations are first projected on a reduced space, and the resulting equations are solved
numerically as a time-marching problem on the reduced space. Therefore, the intrusive schemes require significant modification of the solver whereas the
non-intrusive reduced order model, on the other hand, is entirely data-driven and a surrogate model is generated with a database from a high-fidelity numerical
or experimental dataset. Therefore, the second approach requires minimal changes in the computational solver.

The projection-based intrusive reduced order model often possesses numerical stability issues if the solution manifold is highly nonlinear, requiring a large dimension of the linear subspace used to approximate the solution manifold and increasing the computational cost of the
reduced order schemes. Among several intrusive reduced-order model approaches,
POD-Galerkin-based ROM \cite{STABILE2018273,KaratzasStabileNouveauScovazziRozza2019b,StabileHijaziMolaLorenziRozza2017,stabile2020efficient}, has been very effective in approximating the dynamics in a low dimensional manifold. A
survey of projection-based ROM for parameterized dynamical systems is carried
out by Benner et al.\cite{BennerROM}.  An additional effort is required in the
projection-based intrusive ROM approach to handle the nonlinear term requiring
several hyper-reduction methods \cite{BARRAULT2004667,BDEIM2010,carlberg2013gnat,farhat2015structure}. Since in an intrusive ROM framework, the governing equations are satisfied in the reduced or latent space, this type of ROM is expected to produce accurate prediction even at a sparse training dataset. 

There have been several progresses in non-intrusive
reduced order model in recent times \cite{benner2021system,demo1,demo2019complete,GadallaCianferraTezzeleStabileMolaRozza2020}. For ill-posed problems such as inverse, regression, and classification problems in diverse fields of computational mechanics, as outlined in Schmidhuber et al., \cite{schmidhuber2015deep}, several deep learning (DL) approaches offer effective solutions. Maulik and San \cite{maulik2019subgrid} and Duraisamy et
al.\cite{parish2016paradigm} proposed a turbulence closure model using machine learning. Among other notable applications of deep learning in fluid mechanics problems are the combined proper orthogonal decomposition (POD)
and LSTM network for incompressible flows with spectral proper orthogonal
decomposition (SPOD) of Wang et al. \cite{wang2018model} and the application of
a dimensionality reduction method with DL networks for learning feature dynamics
from noisy data sets in Lui and Wolf \cite{lui2019construction}. As mentioned,
non-intrusive approaches often require a large data set to gain significant
prediction accuracy. LSTM network has been applied to several fields of
computational physics problems such as aeroelastic applications and hydrodynamic
applications by Halder et al. \cite{AHalder2020,halder2023deep}, for the
application in atmospheric turbulence by Rahman et
al.\cite{rahman2019nonintrusive}. However, such approaches, being completely data-driven or black-box methods, require large training datasets computed in the expensive offline stage, and thereby they appear to be ineffective in those application areas where sparse datasets are available. Hence, in the non-intrusive framework, a grey-box approach where the governing dynamics or the parametric space can be learnt from the governing equations in addition to data-driven constraints can circumvent the requirement of a large training dataset. 

In the past century, early work on solving partial differential equations
(PDE) using neural networks starts with Dissanayake and Phan-Thien
\cite{dissanayake1994neural}. With recent advancements in research of neural networks, this
topic got renewed attention with the work of Raissi et al.\cite{CRAISSI2019686}.
Physics-informed neural networks can circumvent the problem of large training
dataset requirements by introducing additional physics-based loss terms. This
physics-based loss term in neural networks can be computed from the governing
equations. Different types of neural networks can be considered in the context of PINN, such as artificial neural networks (ANN) by Raissi et al. \cite{CRAISSI2019686}, Waheed et al.\cite{bin2021pinneik}, Tartakovsky et al. \cite{tartakovsky2020physics} and
Schiassi et al.\cite{schiassi2021extreme}. Similarly, Gao et al. \cite{gao2021phygeonet} and Fang \cite{fang2019physics} coupled convolution neural networks (CNN) with physics constraints. A review of several developments in PINN is summarized by Cuomo et
al.\cite{cuomo2022scientific}. However, there are limited works in Physics Informed Long Short-Term Neural Network (LSTM). Zhang et
al.\cite{cheng2021deep} used a tensor differentiator to determine the derivatives of state space variables to couple the LSTM network with physics information arising from the governing equations and applied to nonlinear-structural problems. PINN usually considers an automatic differential (AD) based approach \cite{baydin2018automatic} for the computation of the gradients. There have been few efforts to use derivatives
based on known numerical approaches such as finite difference, finite-element,
finite volume methods etc. to compute the physics-driven loss-term in the PINN
network. Ranade et al. \cite{RANADE2021113722} proposed a Discretization-net
where finite volume-based numerical residuals are considered in the loss term of
the physics-informed neural network. Similar work by Aulakh et al.
\cite{aulakh2022generalized} coupled physics-informed ANN network with the finite
volume-based discretization of the OpenFOAM solver. The PINN network often takes
more time than the forward solvers due to the large dimensionality of the network output. To reduce this effort the governing equation can be first reduced
using the conventional dimensionality reduction approach, such as Proper Orthogonal Decomposition (POD), and then can be coupled with the
loss equations as shown by Chen et al. \cite{CHEN2021110666} and
Hijazi et al. \cite{hijazi2023pod}. Discretized governing equation augmented
LSTM network is demonstrated for the first time by the author \cite{halder2023deep}, but the detailed comparison of prediction accuracy in the
context of different neural networks and extension of the algorithm to a
spatiotemporal problem will be demonstrated in the present work.

The contribution of the current work is the usage of discretized equations,
projecting them on a reduced space and coupling ANN and LSTM networks to explore
the potential of neural networks where the loss term arises both from the
numerical dataset available and the numerical residual of the discretized
governing equation from a third-party CFD or CSD solvers. In the present work,
although we have coupled the PINN environment with a PyTorch-based external
numerical solver, the motivation of the current work is to bridge the PINN
environment with the existing C++ based open-source solvers for handling complex
geometry and more practical applications as a future endeavour. The current
paper is organized in the following way. First, in \autoref{sec:GE}, the
general formulation of the discretized governing equation is presented, followed by
the reduced-order representation of the discretized equation is discussed. Next,
in \autoref{sec:PINN}, the architecture of the ANN and LSTM network and
their extension to a physics-informed neural network using additional loss
penalty arising from the numerical residual of the reduced order discretized
equations are discussed. Here, we also discuss the software implementations
\cite{demo2023extended} details of the work. Finally, in
\autoref{sec:results}, the proposed approaches are applied in the context of a 2-dof
linear structural equation and a viscous Burgers' equation. The contribution of the current work can be summarized as follows:

\begin{itemize}


\item The current work proposes a novel approach where the existing forward solvers can be used in the PINN framework. Therefore, the solvers can be used for ill-posed and inverse problems. The current work lays the foundation for coupling existing open-source CFD/CSD solvers with the PINN framework for tackling computational mechanics problems involving complex geometry and large-scale problems.

\item Current work proposes discretized governing equations based LSTM-PINN network for unsteady spatio-temporal problems of interest for the first time as per authors' knowledge.

\item Detail studies of prediction and reconstruction capabilities involving several neural networks such as ANN and LSTM and discretized governing equations are carried out.

\item The PINN network often suffers from the large-dimensionality of problems. Therefore, we propose to use the projection-based ROM framework used in \cite{STABILE2018273} in the PINN platform, which is one of the key contributions of the current work.


\end{itemize}




==> Physics_Informed_Neural_Netowork.tex <==
\section{\bf{PINN for Discretized Reduced Order System}}\label{sec:PINN}

In this section, physics informed neural network using the discretized governing equation will be discussed. First, two different types of neural network
architecture such as ANN and LSTM will be briefly introduced in 
\autoref{subsec:NN} followed by the integration with the discretized governing equation in the framework of the physics-informed neural network
\cite{CRAISSI2019686} which will be discussed in \autoref{subsec:ANN-PINN}
and \autoref{subsec:LSTM-PINN}.  

\subsection{Neural Network Architecture}\label{subsec:NN}

ANN formulates a nonlinear functional relationship between the input and output.
In \autoref{eq:18}, $\textbf{f}$ can be considered as input whereas the variable
$\textbf{u}$ can be the output of the neural network and input-output mapping
for a single-layer, ANN network can be written as follows:

\begin{equation}\label{eq:18}
\begin{aligned}
\textbf{u} = f_{\text{act}}(W \textbf{f} + b),
\end{aligned}
\end{equation}

where $f_{act}$ is the nonlinear activation function. %$W$ \GS{also $W$ was used before}  
the weight matrix and
$b$ is the bias vector. In \autoref{eq:18}, the input, $\textbf{f}$ and output $\textbf{u}$ can also
correspond to an unsteady time series problem such as the mass-spring system and
unsteady viscous Burgers' equation. The Eqn.\autoref{eq:18} can be rewritten as \autoref{eq:19}:  

\begin{equation}\label{eq:19}
\begin{aligned}
p_o^{n_t} = f_{act}(W p_i^{n_t} + b),
\end{aligned}
\end{equation}
where ${p_i}^{n_t}$ corresponds to the input of the unsteady problem considered
which is $C_l$ and $C_m$ at $n_t^{th}$ time instant for the pitch-plunge airfoil and
$t$ for the Burgers' equation. Furthermore, $p_o^{n_t}$ corresponds to the output
of the unsteady problem considered which is $h$ and $\alpha$ at $n_t^{th}$ time
instant for the pitch-plunge airfoil and $u$ at all the spatial locations for
the Burgers' equation. However, in Recurrent Neural Networks (RNN), the output,
$p_o^{n_t}$ corresponds to the time history of the input instead of a single time
instant value as shown in \autoref{eq:20}. The other matrix $U_R$ is not present
in the architecture of $ANN$ which is associated with the input from the
previous time steps values and introduces the memory effect in the network
architecture. In different variants of RNN, $h_i^{(n_t)}$ forms a different
functional relationship with previous time instant values of $p_i$. For a simple
RNN network, $h_i^{(n_t)} = p_i^{n_t-1}$   

\begin{equation}\label{eq:20}
\begin{aligned}
p_o^{n_t}=f_\text{act}\left(Wp_i^{n_t}+U_{R} h_i^{(n_t)}+b\right).
\end{aligned}
\end{equation}

The present work considers a variant of the RNN network called a Long Short Term
Memory network (LSTM). A brief introduction to an LSTM cell and the associated
network's input and output architecture will be briefly introduced now, which
will be essential to understand the coupling between the LSTM network with the
discretized PDE-based loss term, a topic of discussion in the following
subsection. However, the advantages of the LSTM network over a simple RNN
network, and the detailed architecture of the LSTM network can be found in
Halder et al. \cite{AHalder2020,halder2023deep}. As mentioned, RNN-type
neural networks require input values associated with a sequence of time
instants. The output corresponds to the last time instant in the input time
sequence. For example, for an input time-series, $[x_1, x_2,x_3 .... x_t]$, corresponding output, $[y_1, y_2,y_3 .... y_t]$ and sequence length of $s$ associated with the input, in the LSTM network, $[x_1, x_2,...x_s]$ corresponds to output
$y_s$. The input of the LSTM forms a tensor structure as shown in
\autoref{fig:Fig1a} where the number of input variables attributed to the third
dimension. For example, for a pitch-plunge airfoil system, the number of input
variables is 2 which are $C_l$ and $C_m$ and for the Burgers' equation, time, $t$
being the only input variable, its dimension is $1$.
Conversely, the output structure forms a matrix as shown in \autoref{fig:Fig1b}
where the second dimension corresponds to the number of output variables. For a
pitch-plunge airfoil system, the number of output variables is 2 which are $h$
and $\alpha$, whereas, for the Burgers' equation the number of output variables
is the number of spatial locations.

However, this input-output structure of both ANN and LSTM networks is adequate
to understand the discretized reduced order system enhanced physics-informed
neural network termed as ANN-DisPINN and LSTM-DisPINN respectively which we will discuss in the following 
\autoref{subsec:ANN-PINN} and \autoref{subsec:LSTM-PINN} .

\begin{figure}[ht] \label{Fig1}
\centering
\begin{subfigure}[b]{0.90\textwidth}
\centering
% \hspace{-3cm}
\subfloat[ Input Tensor of LSTM
]{\label{fig:Fig1a}\includegraphics[width=.60\linewidth]{images/Method_Image/Input_LSTM.png}}
\subfloat[Output of
LSTM]{\label{fig:Fig1b}\includegraphics[width=.35\linewidth]{images/Method_Image/Output_LSTM.png}}
\end{subfigure}
\medskip
\caption{Architecture of an input and output architecture of LSTM}
\label{fig:Fig1}
\end{figure}

\subsection{ANN-DisPINN}\label{subsec:ANN-PINN} In this section,  the discretized
full-order or reduced-order governing equation is employed in the
physics-informed neural network framework. The input and output structure of a
simple ANN and ANN-Network is straightforward. For an unsteady problem, $[x_1,
x_2,x_3,\dots,x_t]$ is the input associated with different time instants and
$[y_1, y_2,y_3,\dots,y_t]$ are the output values corresponding to the inputs.
Hence, a one-to-one correspondence exists between the input and output
formulations associated with each time instant. However, in ANN-DisPINN proposed
here in \autoref{fig:Fig2}, an additional loss penalty is introduced in addition to
the data-driven loss part, which is coming from the discretized governing
equation as shown in \autoref{eq:11} and \autoref{eq:13}. The data-driven and
physics-driven loss functions associated with the pitch-plunge airfoil and
viscous Burgers' equation are as follows:

\begin{equation}\label{eq:21}
\begin{aligned}
MSE_\text{Data} = || y_\text{pred} - y_\text{actual}||_{L2},\\
MSE_\text{burgers} =  || r_\text{burgers} ||_{L2}, \\
MSE_\text{rigid-body} =  || r_\text{rigid-body} ||_{L2},
\end{aligned}
\end{equation}

where, $y_\text{pred}$ is the predicted outcome from \autoref{eq:18} and $y_\text{actual}$
is the benchmark numerical dataset available. The loss terms arising from the
data-driven term $MSE_\text{Data}$ and physics-driven term $MSE_\text{burgers}$
and $MSE_\text{rigid-body}$ need to be minimized to obtain the weight matrix
$W$ and bias vector $b$ as mentioned in \autoref{eq:18} from this
non-convex optimization problem statement which is inherent to the neural network
algorithm. The 2-dof rigid body dynamical system does not require any spatial
reduction whereas, the Burgers' equation is first projected on a reduced basis
followed by residual computation from the reduced discretized equation which
further serves as a loss penalty in the physics-driven loss term of ANN network
as $MSE_\text{burgers-reduced} =  || r_\text{burgers,reduced} ||_{L2}$ 

\begin{figure}[t]
    \centering
    \includegraphics[width=100mm,scale=0.5]{images/Method_Image/ANN_in_PINN.png}
        \caption{Architecture of ANN-DisPINN}
        \label{fig:Fig2}
\end{figure}

%\GS{I don't like }

\subsection{LSTM-DisPINN}\label{subsec:LSTM-PINN}

As shown in \autoref{fig:Fig1a} and \autoref{fig:Fig1b}, the input to the network is
first re-formulated with a sequence length and then it is passed through the
LSTM architecture as shown in \autoref{fig:Fig3a} and \autoref{fig:Fig3b}  to
obtain the $y_\text{pred}$ from the nonlinear functional relationship between the input
and output. It is clear from \autoref{fig:Fig1b}, we only obtain predicted
output from $s^{th}$ time step. The $y_\text{pred}$ is further used to minimize the
loss terms $MSE_\text{Data}$, $MSE_\text{physics, burgers}$ and $MSE_\text{physics,
rigid-body}$ to obtain the weight matrices and bias vectors associated with the
LSTM network. Similarly, for the reduced order discretized system, $MSE_\text{physics,
burgers-reduced}$ should be considered in the physics-driven loss term.  \\

\begin{figure}[ht] 
\centering
\begin{subfigure}[b]{0.90\textwidth}
\centering
% \hspace{-3cm}
\subfloat[ A single LSTM Cell]{\label{fig:Fig3a}\includegraphics[width=.35\linewidth]{images/Method_Image/LSTM_Cell1.png}}
\subfloat[LSTM-PINN
]{\label{fig:Fig3b}\includegraphics[width=.65\linewidth]{images/Method_Image/LSTM_Cell_in_PINN.pdf}}
\end{subfigure}
\medskip
\caption{Architecture of a single LSTM-Cell and Discretized PDE-based LSTM-DisPINN}\label{fig:Fig3}
\end{figure}

The advantages of using the discretized system in the loss-term of the discretized-physics-informed neural networks are summarised below:
\begin{itemize}

  \item The automatic differentiation (AD) based gradient computation \cite{baydin2018automatic} in
  conventional PINN framework requires the spatial coordinates (i.e., Cartesian
  coordinates) and time coordinates as the input to the neural network where the current approach provides a flexible choice of input.  
  \item If a sparse numerical dataset is available to introduce in the
  data-drive loss term of the PINN network, they should comply with the
  numerical derivatives used in the physics-driven loss function, which have
  been used to generate those numerical datasets. However, in the conventional
  PINN framework, the numerical data often does not comply with the AD-based
  derivative resulting in a less accurate prediction.
\end{itemize}

The discretized-physics-based neural network(DisPINN) can be put in the context of a projection-based reduced order model and data-driven approach as shown in \autoref{fig:DisPINN}. The implementation of the ANN-DisPINN and LSTM-DisPINN is carried out in the PyTorch-based PINN platform, PINA \cite{coscia2023physics}. 

\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{images/Method_Image/method_final1.pdf}
        \caption{General framework for different reduced order models and DisPINN approach}
        \label{fig:DisPINN}
\end{figure}

%\GS{let's remember to remake Figure 4; I don't like the orange on blue and the change of color}

